Non-Uniform and Weighted Crossing Gates in Two-Dimensional Sandpiles

Determining whether predicting two-dimensional sandpiles lies in $\mathbf{NC}$ or is $\mathbf{P}$-complete has been open for decades. Moore and Nilsson proved $\mathbf{P}$-completeness for the three dimensional case by encoding Boolean circuits into sandpiles, but this method fails in two dimension due to the impossibility of crossing gates. In this work, we study the existence of crossing gates on non-uniform and weighted grids. We establish an equivalence between uniform weighted crossing gates and a class of simple non-uniform crossing gates, which we call primal. We also exhibit a crossing gate that inherently requires more than one crossing, rather than a single crossing as in standard constructions. Finally, we show that the equivalence between uniform weighted and primal crossings breaks down in more general settings.

==> tikzifieur/damier.tex <==
% damier-odd
\matrix[table,] (damier-odd){
\node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0};\\
\node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4};\\
\node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0};\\
\node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4};\\
\node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0};\\
};

% damier-even
\node[right = 2mm of damier-odd] (damier-odd-top-arr) {$\xmapsto[]{T}$};
\matrix[table,right = 2mm of damier-odd-top-arr,] (damier-even){
\node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4};\\
\node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0};\\
\node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4};\\
\node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0};\\
\node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4}; & \node[] {0}; & \node[fill=black!57.14,text=white] {4};\\
};



==> tikzifieur/moore-gates.tex <==
% gate-wire
\matrix[table,] (gate-wire){
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[fill=black!100.00,text=white](gate-wire-0-2) {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white](gate-wire-4-2) {5};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
};
\draw[ain] (gate-wire-0-2) -- +(left:6mm);
\draw[aout] (gate-wire-4-2) -- +(right:5.5mm);
\node[below=0 of gate-wire,] {Fil};

% gate-turn
\matrix[table,right= of gate-wire] (gate-turn){
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white](gate-turn-3-0) {5}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0};\\
\node[fill=black!100.00,text=white](gate-turn-0-3) {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
};
\draw[ain] (gate-turn-0-3) -- +(left:6mm);
\draw[aout] (gate-turn-3-0) -- +(up:5.5mm);
\node[below=0 of gate-turn,] {Tournant};

% gate-dup
\matrix[table,right= of gate-turn] (gate-dup){
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white](gate-dup-4-1) {5};\\
\node[fill=black!100.00,text=white](gate-dup-0-2) {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white](gate-dup-4-3) {5};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
};
\draw[ain] (gate-dup-0-2) -- +(left:6mm);
\draw[aout] (gate-dup-4-1) -- +(right:5.5mm);
\draw[aout] (gate-dup-4-3) -- +(right:5.5mm);
\node[below=0 of gate-dup,] {Duplication de signal};

% gate-or
\matrix[table,below= of gate-wire] (gate-or){
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[fill=black!100.00,text=white](gate-or-0-1) {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white](gate-or-4-2) {5};\\
\node[fill=black!100.00,text=white](gate-or-0-3) {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
};
\draw[ain] (gate-or-0-1) -- +(left:6mm);
\draw[ain] (gate-or-0-3) -- +(left:6mm);
\draw[aout] (gate-or-4-2) -- +(right:5.5mm);
\node[below=0 of gate-or,] {Porte OU};

% gate-and
\matrix[table,right= of gate-or] (gate-and){
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[fill=black!100.00,text=white](gate-and-0-1) {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!80.00,text=white] {4}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white](gate-and-4-2) {5};\\
\node[fill=black!100.00,text=white](gate-and-0-3) {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
};
\draw[ain] (gate-and-0-1) -- +(left:6mm);
\draw[ain] (gate-and-0-3) -- +(left:6mm);
\draw[aout] (gate-and-4-2) -- +(right:5.5mm);
\node[below=0 of gate-and,] {Porte ET};

% gate-diode
\matrix[table,right= of gate-and] (gate-diode){
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0};\\
\node[fill=black!100.00,text=white](gate-diode-0-2) {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!80.00,text=white] {4}; & \node[fill=black!100.00,text=white](gate-diode-4-2) {5};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
};
\draw[ain] (gate-diode-0-2) -- +(left:6mm);
\draw[aout] (gate-diode-4-2) -- +(right:5.5mm);
\node[below=0 of gate-diode,] {Diode};

% gate-cross-b
\matrix[table,below= of gate-or] (gate-cross-b){
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
};
\node[below=0 of gate-cross-b,cross] {Porte de croisement \\ (-1 dans la 3~ème dimension)};

% gate-cross-0
\matrix[table,right= of gate-cross-b] (gate-cross-0){
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white](gate-cross-0-2-0) {5}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[] {0};\\
\node[fill=black!100.00,text=white](gate-cross-0-0-2) {5}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[fill=black!100.00,text=white](gate-cross-0-4-2) {5};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white](gate-cross-0-2-4) {5}; & \node[] {0}; & \node[] {0};\\
};
\draw[ain] (gate-cross-0-0-2) -- +(left:6mm);
\draw[ain] (gate-cross-0-2-0) -- +(up:6mm);
\draw[aout] (gate-cross-0-4-2) -- +(right:5.5mm);
\draw[aout] (gate-cross-0-2-4) -- +(down:5.5mm);
\node[below=0 of gate-cross-0,cross] {Porte de croisement \\ (0 dans la 3~ème dimension)};

% gate-cross-a
\matrix[table,right= of gate-cross-0] (gate-cross-a){
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[fill=black!100.00,text=white] {5}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {0};\\
};
\node[below=0 of gate-cross-a,cross] {Porte de croisement \\ (1 dans la 3~ème dimension)};



==> tikzifieur/neig-inter.tex <==
% neig-inter-1
\matrix[table,] (neig-inter-1){
\node[] {0}; & \node[] {0}; & \node[fill=black!14.29,text=black] {1};\\
\node[] {0}; & \node[fill=blue!30] {-5}; & \node[] {0};\\
\node[fill=black!14.29,text=black] {1}; & \node[fill=black!14.29,text=black] {1}; & \node[fill=black!14.29,text=black] {1};\\
\node[] {0}; & \node[fill=black!14.29,text=black] {1}; & \node[] {0};\\
};
\node[below=0 of neig-inter-1,] {$\nei_5$};

% neig-inter-n
\matrix[table,right=of neig-inter-1] (neig-inter-n){
\node[] {0}; & \node[] {0}; & \node[fill=black!25.00,text=black] {1}; & \node[] {0}; & \node[] {0}; & \node[] {0}; & \node[] {$\cdots$}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[fill=blue!30] {-}; & \node[fill=black!25.00,text=black] {1}; & \node[fill=black!25.00,text=black] {1}; & \node[fill=black!25.00,text=black] {1}; & \node[fill=black!25.00,text=black] {1}; & \node[] {$\cdots$}; & \node[fill=black!25.00,text=black] {1}; & \node[fill=black!25.00,text=black] {1};\\
\node[fill=black!25.00,text=black] {1}; & \node[] {0}; & \node[fill=black!25.00,text=black] {1}; & \node[] {0}; & \node[fill=black!25.00,text=black] {1}; & \node[] {0}; & \node[] {$\cdots$}; & \node[fill=black!25.00,text=black] {1}; & \node[] {0};\\
};
\node[below=0 of neig-inter-n,] {$\nei_6$};



==> tikzifieur/neig-weighted.tex <==
% neig-weighted-1
\matrix[table,] (neig-weighted-1){
\node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[fill=blue!30] {-5}; & \node[fill=black!14.29,text=black] {1};\\
\node[fill=black!28.57,text=black] {2}; & \node[] {0}; & \node[fill=black!28.57,text=black] {2};\\
};
\node[below=0 of neig-weighted-1,] {$\nei_1$};

% neig-weighted-2
\matrix[table,right = of neig-weighted-1] (neig-weighted-2){
\node[] {0}; & \node[fill=black!28.57,text=black] {2}; & \node[] {0};\\
\node[fill=black!14.29,text=black] {1}; & \node[fill=blue!30] {-5}; & \node[fill=black!14.29,text=black] {1};\\
\node[] {0}; & \node[fill=black!14.29,text=black] {1}; & \node[] {0};\\
};
\node[below=0 of neig-weighted-2,] {$\nei_2$};

% neig-weighted-3
\matrix[table,right = of neig-weighted-2] (neig-weighted-3){
\node[] {0}; & \node[fill=black!28.57,text=black] {2}; & \node[] {0};\\
\node[fill=black!14.29,text=black] {1}; & \node[fill=blue!30] {-8}; & \node[fill=black!14.29,text=black] {1};\\
\node[] {0}; & \node[fill=black!14.29,text=black] {1}; & \node[fill=black!42.86,text=black] {3};\\
};
\node[below=0 of neig-weighted-3,] {$\nei_3$};

% neig-weighted-4
\matrix[table,right = of neig-weighted-3] (neig-weighted-4){
\node[] {0}; & \node[] {0}; & \node[] {0};\\
\node[] {0}; & \node[fill=blue!30] {-2}; & \node[fill=black!14.29,text=black] {1};\\
\node[] {0}; & \node[fill=black!14.29,text=black] {1}; & \node[] {0};\\
};
\node[below=0 of neig-weighted-4,] {$\nei_4$};



==> tikzifieur/no-inter.tex <==
% no-inter
\matrix[table,] (no-inter){
\node[fill=blue!30] {-}; & \node[fill=black!14.29,text=black] {1}; & \node[fill=black!14.29,text=black] {1}; & \node[] {$\cdots$}; & \node[fill=black!14.29,text=black] {1}; & \node[] {0};\\
\node[fill=black!14.29,text=black] {1}; & \node[] {0}; & \node[] {0}; & \node[] {$\cdots$}; & \node[] {0}; & \node[] {0};\\
};


